DeepFry: Identifying Vocal Fry Using Deep Neural Networks

Vocal fry or creaky voice refers to a voice quality characterized by irregular glottal opening and low pitch. It occurs in diverse languages and is prevalent in American English, where it is used not only to mark phrase finality, but also sociolinguistic factors and affect. Due to its irregular periodicity, creaky voice challenges automatic speech processing and recognition systems, particularly for languages where creak is frequently used. This paper proposes a deep learning model to detect creaky voice in fluent speech. The model is composed of an encoder and a classifier trained together. The encoder takes the raw waveform and learns a representation using a convolutional neural network. The classifier is implemented as a multi-headed fully-connected network trained to detect creaky voice, voicing, and pitch, where the last two are used to refine creak prediction. The model is trained and tested on speech of American English speakers, annotated for creak by trained phoneticians. We evaluated the performance of our system using two encoders: one is tailored for the task, and the other is based on a state-of-the-art unsupervised representation. Results suggest our best-performing system has improved recall and F1 scores compared to previous methods on unseen data.

==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/bibtoadd.tex <==


@article{ishi2007method,
  title={A method for automatic detection of vocal fry},
  author={Ishi, Carlos Toshinori and Sakakibara, Ken-Ichi and Ishiguro, Hiroshi and Hagita, Norihiro},
  journal={IEEE transactions on audio, speech, and language processing},
  volume={16},
  number={1},
  pages={47--56},
  year={2007},
  publisher={IEEE}
}

@article{kane2013improved,
  title={Improved automatic detection of creak},
  author={Kane, John and Drugman, Thomas and Gobl, Christer},
  journal={Computer Speech \& Language},
  volume={27},
  number={4},
  pages={1028--1047},
  year={2013},
  publisher={Elsevier}
}

%%%%checking code
@inproceedings{white2021optimizing,
  title={Optimizing an automatic creaky voice detection method for Australian English-speaking females},
  author={White, Hannah and Penney, Joshua and Gibson, Andy and Szakay, Anita and Cox, Felicity},
  booktitle={INTERSPEECH (22nd: 2021)},
  pages={1384--1388},
  year={2021},
  organization={International Speech Communication Association (ISCA)}
}

@article{devaraj2021modelling,
  title={Modelling of Amplitude Modulated Vocal Fry Glottal Area Waveforms Using an Analysis-by-Synthesis Approach},
  author={Devaraj, Vinod and Aichinger, Philipp},
  journal={Applied Sciences},
  volume={11},
  number={5},
  pages={1990},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/conclusions.tex <==
\section{Conclusions}
In this work, we present a system composed of an encoder and a classifier for creak detection. We investigated two types of encoders that work on the raw wave: (i) \algoname~ which is a small network with large receptive field and (ii) \hubert~which is a state-of-the-art encoder that was pre-trained on a lot of data and has a lot of parameters. Results suggest, that both of our implementations, achieve higher recall and F1 scores than the methods we compared to. Furthermore, it is evident that while \algoname~had better results on the test set of \textit{Nuclear} dataset, \hubert~had higher recall and F1 scores on datasets from different distribution. We believe this is due to the vast amount \hubert~was trained on. Thus, it remains for future work to investigate the effect of training with more data on \algoname.



\section{Acknowledgements}
Y. Segal is sponsored by the Ministry of Science \& Technology, Israel.




==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/dataset.tex <==
\section{Datasets}\label{dataset}
Three datasets of American English connected speech were annotated for creaky voice. 
The first two datasets investigated the relationship between information structure and the realization of nuclear and prenuclear pitch accents in American English.
%Data Set 1 investigated the realization of the nuclear pitch accent, which is the final pitch accent within an intonational phrase; Data Set 2 investigated the realization of the prenuclear pitch accent, which is any pitch accent preceding the nuclear pitch accent in the same intonational phrase.
%\todo{check on naming of Data Set 1 and Data Set 2. Maybe we capitalize them; would it be better to refer to them as Nuclear and Prenuclear or is that too weird for the average reader? }
The third dataset is the American English subset of the ALLSSTAR corpus (Archive of L1 and L2 Scripted and Spontaneous Transcripts and Recordings)\cite{bradlow2010allsstar}. Throughout the paper, the datasets are denoted as \textit{Nuclear}, \textit{Prenuclear} and \textit{ALLSSTAR}, respectively.

The \textit{Nuclear} and \textit{Prenuclear} datasets contain speech from 32 native speakers of American English (\textit{Nuclear}: 16 female, 16 male; \textit{Prenuclear}: 11 female, 21 male), and the \textit{ALLSSTAR} dataset contained speech from 14 native speakers of American English (7 female, 7 male).
All participants were university-aged students.
%Northwestern University students in Evanston, IL, USA. 
%The recordings were made at Northwestern University
%The \textit{Nuclear} dataset had 16 female and 16 male speakers; %and the ages ranged from 18 to 21 (median = 19). 
% The recordings were made in late 2018. 
%6 participants were from the Northeast, 10 from the Midwest, 5 from the South, 6 from California, and 5 from elsewhere in the US.
%The \textit{Prenuclear} dataset had 11 female and 21 male speakers, and the ages ranged from 18 to 22 (median = 20). 
% The recordings were made in late 2018 and early 2019. 
%13 participants were from the Northeast, 11 from the Midwest, 6 from the South, and 2 from California.
%The \textit{ALLSSTAR} dataset had 7 female and 7 male speakers, and the ages ranged from 18 to 21 (median = 19).
% The recordings were made in 2010 and 2011. %\todo{verify with Ann Bradlow? original ALLSSTAR team is from 2010-2011 according to website}
%5 participants were from the Northeast, 6 from the Midwest, 2 from the South, and 1 from California.
%\todo{if needed, remove location info}

In the \textit{Nuclear} and \textit{Prenuclear} datasets, participants read aloud a series of three-sentence stories. 
Only the final `target' sentence was used in the present study of creak.
%(The first two sentences of the story set up the information structure of a noun in the target sentence.)
% Each target sentence had the following syntactic and metrical structure: determiner (one syllable), subject noun (two syllables, stress-initial), verb (one syllable), determiner (one syllable), object noun (three syllables, stress-initial), and a final phrase that was either an adverbial phrase (e.g. `there'), a prepositional phrase (e.g., `for it'), or a short relative clause (e.g., `she had'). 
% When constructing the sentence, nouns and verbs with mostly sonorant segments were prioritized. 
%but voiceless obstruents were not entirely avoided in the full sentence. 
Each participant read all 20 target sentences (within a unique story) in a randomized order in four separate blocks. Only the first two blocks were analyzed. 
Block 1 was read in a neutral speaking style and block 2 in a lively speaking style. 
The \textit{ALLSSTAR} dataset contained readings of the first ten Hearing in Noise Test sentences in the ALLSSTAR HINT1 subset. 
The recordings in all three datasets were made at Northwestern University in a soundproof booth with a sampling rate of 22.05 kHz; all recordings were resampled to 16 kHz for the experiments. %\todo{maybe check with Ann Bradlow to see that they also recorded in the speech lab?}
Sentences which contained a speech disfluency were removed from the analysis. As a result, 1195 sentences were available for analysis in the \textit{Nuclear} dataset, 1200 sentences in the \textit{Prenuclear} dataset, and 140 sentences in the \textit{ALLSSTAR} dataset . 

%  For the \textit{Nuclear} and \textit{Prenuclear} datasets, a median of 2 sentences were removed from each file. 
% In total, 1195 sentences were available for analysis in the \textit{Nuclear} dataset and 1200 sentences in the \textit{Prenuclear} dataset. 
% No sentences were removed from the \textit{ALLSSTAR} dataset; 140 sentences were available for analysis.

% For Data Set 1, the mean percentage creak across speakers and in sonorant intervals only was 25.49\% (SD = 11.10\%, range = 5.55\% to 48.86\%). For Data Set 2, it was 22.92\% (SD = 11.60\%, range = 2.74\% to 61.31\%), and for Data Set 3, it was 14.58\% (SD = 6.40\%, range = 0.00\% to 25.50\%). (Though Data Set 3 differs from Data Sets 1 and 2 in generation, the reading material also differed slightly. The annotated creak in the first two data sets came from the final sentence in a short story; the data in Data Set 3 came from a sentence read in isolation. More research would be necessary to determine the precise source of this difference.)
The \textit{Nuclear} dataset was divided into train (20 participants - about 24 minutes), validation (6 participants - about 6 minutes), and test (6 participants - about 8 minutes) folds where each fold contained an equal number of male and female participants. The \textit{Prenuclear} and \textit{ALLSSTAR} datasets were used for evaluation. 


%%% creak annotation
\subsection{Annotation}
%The target sentence of the first 40 trials from each participant was annotated for voice quality. 
%The target sentence was annotated for voice quality; for the `nuclear final' data set, all 80 trials were annotated; for the `nuclear + final phrase' and 'prenuclear + final phrase' data sets, the first 40 trials for each participant were annotated.
To annotate the data, the transcripts were submitted to the Montreal Forced Aligner (MFA) for word- and phone-level alignments using the default American English pronunciation dictionary and acoustic model \cite{mcauliffe2017montreal}.
From these boundaries, we annotated the target sentences using two voice quality labels: modal or creaky voice, which are reasonably well-defined on sonorant segments.
%The first run was used to obtain utterances boundaries and was refined if needed. 
%The second time, the aligner was used to receive a word and phone-level alignment of the sentences. %During annotation, the utterances boundaries and refined them, if needed.were checked and refined, if needed. These were then submitted to the Montreal Forced Aligner  using the default American English pronunciation dictionary and acoustic model\cite{mcauliffe2017montreal}.  %This resulted in a word and phone-level alignment of the sentence.
% Furthermore, two voice quality labels were used for the annotation: modal or creaky voice. 
% Modal and creaky voice could be reasonably well-defined on sonorant segments.
%; as voice quality was either undefined or ill-defined on obstruent consonants, obstruents inherited the modal or creaky label of its syllable. 
% For evaluation purposes, obstruents were assigned the default `modal' voice label, which effectively meant `not creak'.
%for evaluation purposes.
%In the annotation itself, 
%For example, if an obstruent was word-medial and intervocalic, it was grouped with the following sonorant interval as the syllable onset.
%Word-final obstruents were grouped with the preceding sonorant as the syllable coda. 
An interval was labeled as modal voice if a visible pitch track was present in Praat over a sonorant region, and one of the following two scenarios held true: 1) the interval had audible modal voice quality (conveyed audible pitch, had a similar `smooth' voice quality as other prototypical modal regions), or 2) there was visible evidence of modal voicing from glottal pulses in the spectrogram or periodicity in the waveform.
%Evidence of periodicity in waveform included at least three cycles with a duration of 2 to 20 ms each (corresponding to an F0 between 50 to 500 Hz).
An interval was labeled as creak if no visible pitch track was present over a sonorant region in Praat and the above criteria for modality were not met. %Note that this is a coarse usage of creaky voice. \todo{read Keating/Garellek - I think creak is the umbrella term for other more specific cases of fry, pressed voice, etc, so we should be ok. I think this does include breathy voice though.}
%Following annotation, the transcripts were resubmitted to the
The utterance boundaries were refined during annotation and resubmitted to the MFA for a more precise phone-level alignment. 
We note, that in our labeling process, only unvoiced phonemes could not be tagged as creak.

%WE SHOULD SAID SOMETHING ABOUT IT -> We claimed in our study that only voiced phonemes can be labelled as creaky. \todo{say something about what? / where should we say this? ohh -- did we report any evaluations over *all* the speech? Yeah, so we should make sure we run our evaluations over just the sonorant segments?}
%we changed the labels as just if the phonemes where Sonorants it can be call creak
%I changed the R script to label the other data as not creaky...
%Hmm so any [ptkbdgs] etc would be modal? yes
%Ahh ok 


==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/experiments.tex <==

\section{Experiments}
% \todo{Well I was sure we need to fill up space so I added this :D can remove it altogether lol}
In this section, we present the results of our method. We begin by describing the hyper-parameters used to train our model. Then, we describe the measures used to evaluate our method and the adjustment we made to consider the different frame-rate of each method. Following that, we present ablation experiments of our model. We conclude this section by comparing our models to other methods on various unseen datasets and our test set.
We trained \algoname~for 14 epochs, with an Adam optimizer, a learning rate of 0.001, a dropout of 0.1 and batch size 16. 
\hubert~was trained for six epochs, with an Adam optimizer, a learning rate of 0.001, and a batch size of 16. Both models were trained on the \textit{Nuclear} dataset, and for both of them, we stipulated that the classification of a given frame was creak only if the frame was also predicted as voiced at inference time. 
\subsection{Evaluation method}
We evaluated all models using Precision (P), Recall (R) and F1 measures. Precision is defined as the number of creaky frames correctly classified by the algorithm divided by the total number of frames classified as creaky by the algorithm. Recall is defined as the number of creaky frames correctly classified by the algorithm divided by the total number of ground truth creaky frames. The F1 measure is defined as $F1 = {2PR}/{(P+R)}$.

Furthermore, our models, and the models we compare to, output predictions at a different frame-rate. Thus, for a fair comparison, all models classification was evaluated for a 20 ms frame-rate/window.


\subsection{Baseline model}\label{sec:baselines}

Our  baseline model (referred to as the `Praat baseline') used heuristics to detect the onset or offset of creaky voice for a given interval of speech \cite{boersma1993accurate}.
The heuristic operated on the assumption that modal voice could be detected by trackable numeric pitch values, and creaky voice would be associated with an undefined pitch value in Praat.
%Pitch values were first extracted from a given speech interval using Praat's autocorrelation method with 
The script either moved \textit{start-to-end} or \textit{end-to-start} through Praat-extracted pitch values (time step = 0.15 s; pitch range = 50 to 350 Hz). 
When moving start-to-end, the script assumed modal voice was present until it encountered a sequence of undefined pitch values in frame $n$ and frame $n+2$.
When moving end-to-start, the script assumed creaky voice was present until it encountered a sequence of numeric pitch values in frame $n$ and frame $n-2$.
%This model was designed under the assumption that .
For intervals where the speech interval was not fully sonorant, creaky voice was frequently confused with a voiceless segment. 


% (The original model was developed on the assumption that no voiceless segments were present.)
%First, pitch values were extracted from a given speech interval using Praat's autocorrelation method with a time step of 0.15 s and a pitch range of 50 to 350 Hz. 
%The script either moved start-to-end or end-to-start through the Praat-extracted pitch values. 
%The start-to-end script identified the first sequence of undefined pitch values in frame $n$ and frame $n+2$. 
%The script assumed that creak started at frame $n$ and persisted to the end of the interval.
%The end-to-start script identified the first sequence of two numeric pitch values at frame $n$ and frame $n-2$. 
%This script assumed that creak, if present, would occur at the end of the interval.

For the \textit{Nuclear} and \textit{Prenuclear} datasets, the start-to-end mode was used for the first three regions of the target sentence, namely the subject noun phrase, the verb and following determiner, and the object noun phrase. The final phrase and the full sentences in the \textit{ALLSSTAR} dataset were analyzed using the end-to-start mode. 
%\todo{I could easily rerun this on a simpler set of intervals...like two intervals per sentence instead of 4}
%For the \textit{ALLSSTAR} dataset, the full sentence was submitted for analysis using the end-to-start mode.
%The start-to-end script was run on the first three of four intervals of sentences in the \textit{Nuclear} and \textit{Prenuclear} datasets. 
%This script was run on the final phrases of sentences of the \textit{Nuclear} and \textit{Prenuclear} datasets, as well as the full sentences in the \textit{ALLSSTAR} dataset. 

% \todo{\cite{kane2013improved} ...Voice analysis toolkit (VAT) perform... feature extraction and then pass the features to a binary decision tree which outputs the final prediction. We used their framework 
% \footnote{\scriptsize\url{https://github.com/jckane/Voice_Analysis_Toolkit}}   
% to run predictions on our test set.}




% is the Voice Analysis Toolkit\footnote{\scriptsize\url{https://github.com/jckane/Voice_Analysis_Toolkit}}. They used specially designed acoustic features relevant to creaky voice as input to a shallow artificial neural networks

% the detection is based on a combination of new and existing acoustic features relevant to creaky voice which are used as input features to a artificial neural networks based classifier, which has been trained on a wide range of speech
	       
% specially designed acoustic features from the excitation and residual of the linear prediction filtering analysis of the speech and other acoustic features. 

%and would otherwise have modal voice.
%This system works slightly better when no voiceless segments are at the beginning of an interval. 
%For the final phrase interval, the script moved backwards through the Praat pitch values, and 
%This model resulted in three possible output types per interval: fully modal, fully creaky, or modal followed by creaky. 





%Praat Auto Creak using Heuristics 

%right2left

%This system starts from the end of an interval and looks for the first sequence of two numeric pitch values at frame n and frame n-2 (the system moves backwards through the signal).

%The system basically assumes that if creak is going to occur, it will occur at the end of an interval (and Praat returns an "--undefined-- Hz" value), and then it looks for the first instance of modal voice (numeric pitch value). 

%Update: I am running the script on the final word and the final phrase (sometimes multiple words) separately, but technically, we could choose an interval of any length. 

%This system works better on the final phrase because the phrase has several voiceless segments right at the beginning.



%left2right.praat: markCreakyVoice


\begin{table}[h]
  \caption{The contribution of the classification heads for final predictions. Precision (P), recall (R), and F1 scores on the \textit{Nuclear} test set. Predictions are evaluated at a 20 ms frame-rate.}
  \label{tab:results_model1}
  \centering
%   \resizebox{\columnwidth}{!}{
  \begin{tabular}{@{\extracolsep{0.1pt}}lcccccc}
  \toprule
    \multirow{2}{*}{Models}& \multicolumn{3}{c}{Classification heads} &   \multirow{2}{*}{P} & \multirow{2}{*}{R} & \multirow{2}{*}{F1}   \\
    \cmidrule(r){2-4} 
    & Creak & \!\!\!Voice\!\!\! & Pitch & & \\
    \midrule
 \multirow{ 4}{*} \algoname&   $\surd$&&  &  \textbf{68.35}  &  69.64 &  68.99  \\
&   $\surd$&\!\!\!\!$\surd$\!\!\!\!& &  66.01 & 73.42 &  69.52 \\
   &   $\surd$&\!\!\!\!\!\!\!&$\surd$ & 67.30  &  69.67 & 68.46 \\
     &$\surd$&\!\!\!\!$\surd$\!\!\!\!&$\surd$& 67.43  &  \textbf{76.27}    &  \textbf{71.57}\\
\hline
\multirow{ 4}{*} \hubert &  $\surd$&&  & 68.65  &64.97  & 66.76  \\
  &   $\surd$ &\!\!\!\!$\surd$\!\!\!\!&&  \textbf{69.29} &64.52 &  66.82\\
    &   $\surd$&\!\!\!\!\!\!\!\!&$\surd$ & 68.07 & 68.66 & 68.36 \\
   &$\surd$&\!\!\!\!$\surd$\!\!\!\!&$\surd$& 68.74 &  \textbf{69.19}  & \textbf{68.96}   \\
     
    \bottomrule
  \end{tabular}
%   }
\end{table}


\begin{table*}[h]
  \centering
  \setlength{\tabcolsep}{1em}
\captionsetup{width=1.8\columnwidth}
% \renewcommand{\textwidth}
% \resizebox{\linewidth}{!}{
% \renewcommand{\arraystretch}{2}

\caption{Comparison to other methods. Precision (P), Recall (R), and F1 scores on different phonetic subsets of the test set of the \textit{Nuclear} dataset. Sonorants include vowels, glides, liquids, and nasals. Metrics are reported as percentages. Predictions are evaluated at a 20 ms frame-rate.}
%   \resizebox{\textwidth}{!}{%
% \begin{tabulary}{0.75\textwidth}{l ccc ccc ccc}
\begin{tabular}{l ccc ccc ccc}
      \toprule
      \multirow{ 2}{*}{Models}    & \multicolumn{3}{c}{Vowels}  & \multicolumn{3}{c}{Sonorants} & \multicolumn{3}{c}{All}     \\
      \cmidrule(r){2-4}   \cmidrule(r){5-7}   \cmidrule(r){8-10}

       & P & R & F1      & P  & R  & F1     & P & R & F1     \\
    \midrule
    
Praat baseline &  59.66 &  59.21 & 59.43  &  60.07 & 60.60 & 60.33  & 32.93 &  60.60 & 42.67 \\
Kane \emph{et al.} \cite{kane2013improved} & \textbf{86.63}  & 30.14  & 44.72   &  \textbf{87.53}  &  28.53 &43.03  &  \textbf{75.98} &  28.53  &  41.48 \\

\algoname &  81.76   &   \textbf{75.71}  & \textbf{78.62} &  82.20  &   \textbf{76.27}  &  \textbf{ 79.12}  & 67.43  & \textbf{ 76.27}    &   \textbf{71.57}  \\
\hubert &  78.99    & 68.33 & 73.28&  79.69 &   69.19   & 74.07   & 68.74 &  69.19   & 68.96   \\
    \bottomrule
\end{tabular}
% \end{tabulary}
% }
\label{tab:compare_nuc}
\end{table*}


%  second
\begin{table*}[h]

\captionsetup{width=1.8\columnwidth}
% \captionsetup{width=\textwidth}
  \centering
    % \resizebox{\textwidth}{!}{%
    \caption{Evaluation on unseen data. Precision (P), recall (R), and F1 scores on different phonetic subsets of the \textit{Prenuclear} and \textit{ALLSSTAR} datasets. Sonorants include vowels, glides, liquids, and nasals. Metrics are reported as percentages. Predictions are evaluated at a 20 ms frame-rate.}
\begin{tabular}{llccccccccc}
% \captionsetup{width=\cwidth}

    \toprule
       \multirow{ 2}{*}{Dataset}   &\multirow{ 2}{*}{Models}  & \multicolumn{3}{c}{Vowels} &  \multicolumn{3}{c}{Sonorants} & \multicolumn{3}{c}{All}    \\
        \cmidrule(r){3-5}   \cmidrule(r){6-8}   \cmidrule(r){9-11}
        &   &  P   & R   & F1      & P  & R  & F1     & P & R & F1    \\
    \midrule

   \multirow{ 4}{*}{\textit{Prenuclear}}&  Praat baseline\!\!& 44.01    &51.99 & 47.67 &  46.59    &  54.89   & 50.40 &  25.52    & 54.89  & 34.84\\
& Kane \emph{et al.} \cite{kane2013improved}\!\!&  \textbf{81.14}  & 47.58  & 59.99 &  \textbf{80.32} & 43.07 & 56.07      & 66.51 & 43.07   & 52.28 \\
& \algoname &    74.65   &     \textbf{77.50}      &    76.05      &    74.31        &   76.51      &    75.39    &     61.16      &   76.51     &  67.98     \\ 
& \hubert &    78.97   &  77.05 & \textbf{78.00} &  79.83 &   \textbf{78.24}  & \textbf{ 79.02}   & \textbf{69.53}  &  \textbf{78.24} &  \textbf{73.63}  \\
 \hline
    \multirow{ 4}{*}{\textit{ALLSSTAR}}&  Praat baseline\!\!&   85.34 &38.90 & 53.44 & 84.89 &  38.47  &52.95 & 26.60  &  38.47  &31.45\\
 & Kane \emph{et al.} \cite{kane2013improved}& \textbf{97.15}  &  36.50  & 53.06  &   \textbf{97.39} & 34.02 &  50.42 & \textbf{90.03} & 34.02  & 49.38\\
 & \algoname &   94.06     &   55.23      &  69.59       &    93.27        &   52.23      &       66.96 &    77.20       &   52.23     &   62.30    \\
&\hubert &   75.86   & \textbf{71.37} & \textbf{73.55} & 76.94  &    \textbf{70.33}  &  \textbf{73.49} & 66.74  & \textbf{70.33}     &    \textbf{68.49} \\
    \bottomrule
\end{tabular}
% }

\label{tab:unseen}
\end{table*}
\subsection{Ablation}
We begin the experiments by analyzing the contribution of each additional task to the final detection of creak. To do so, we trained  \algoname~and \hubert~with the following settings: (i) only with creak head (ii) creak head and voice head (iii) creak head and pitch head (iv) with creak, voice, and pitch heads. 

Results are shown in Table \ref{tab:results_model1}, where each row represents a different experiment setting. Interestingly, it can be seen that each model benefits differently from each auxiliary task. 
% While \algoname~ presents a higher F1 value in experiment (2) compared to experiment (1) and (3), \hubert has a higher F1 value in experiment (3) compared to (1) and (2). Finally, suited to multi-task learning, the performance of each model on the final combination of the tasks, leads to an increased performance compared to training on each task individually. 
By inspecting the F1 score, we can see that while \algoname~benefits more from the voice detection head than the pitch detection head, \hubert~presents higher performance with the pitch head. 
Finally, although training with each task individually does not necessarily significantly affect the performance, training with the combination of auxiliary tasks leads to increased performance.
% necessarily
% auxiliary
% \todo{choose phrasing, the preceding/following}\\

% First, we show the contribution of each classification head of Model 1 in Table \ref{tab:results_model1}. Each row represents a different training setting where we train the model without the task of voice or pitch. The last row represents the final model with all three tasks. \todo{choose phrasing, the preceding/following}\\

% First, we evaluated the contribution of each one of the additional tasks for model1 training. 
% Table \ref{tab:results_model1} presents results where we trained Model 1 in four fashions, where first we trained the model to classify frames only as creak/ non-creak. Then we add additional tasks of voice/unvoiced classification or pitch threshold classification. Finally, the last model combines all previous tasks.

% The results suggest that adding both voice and creaky classifiers improve the results over using only creaky classifier. Although, the model with creaky and pitch classifiers shows close F1-score to the model with all the three classifiers, its std values are higher, suggesting that the best model is the one with all the three classifiers.





% \begin{table}[h]
%   \caption{Analysis of per-task \todo{evaluation/contribution} to creak detection. Precision (P), recall (R), and F1 scores on the test set of the \textit{Nuclear} dataset with different multi-tasks training. Metrics are reported as percentages. Predictions are evaluated at a 20 ms frame-rate.}
%   \label{tab:results_model1}
%   \centering
% %   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{@{\extracolsep{4pt}}llccc}
%   \toprule
%     & Tasks &   P & R & F1   \\
%     \midrule
%  \multirow{ 4}{*} \algoname&   creak  &  \textbf{68.35}  &  69.64 &  68.99  \\
% &   creak +  voice &  66.01 & 73.42 &  69.52 \\
%   &   creak + pitch & 67.30  &  69.67 & 68.46 \\
%      &\!\!creak+voice+pitch\!\!& 67.43  &  \textbf{76.27}    &  \textbf{71.57}\\
% \hline
% \multirow{ 4}{*} \hubert &  only creak  & 68.65  &64.97  & 66.76  \\
%   &   creak + voice &  \textbf{69.29} &64.52 &  66.82\\
%     &   creak + pitch & 68.07 & 68.66 & 68.36 \\
%   &\!\!creak+voice+pitch\!\!& 68.74 &  \textbf{69.19}  & \textbf{68.96}   \\
     
%     \bottomrule
%   \end{tabular}
% %   }
% \end{table}



\subsection{Comparison to previous works}
 
% \todo{why we didn't compare to other baselines? we should mention here? or in the baselines section?}\\

We now turn to compare our methods to previous works. We compared \algoname~and \hubert~to the baseline model presented in \secref{sec:baselines} on the test set of the \textit{Nuclear} dataset. We also compared to the model was proposed by Kane \emph{et al.} \cite{kane2013improved}\footnote{We use the open-source framework - Voice Analysis Toolkit \scriptsize\url{https://github.com/jckane/Voice_Analysis_Toolkit}}. We found no other implementations or a detailed enough description of the work mentioned in  \secref{sec:intro}.

Table \ref{tab:compare_nuc} presents the comparison for different subsets of phonemes, to gain a deeper understanding of the results. The first column, \textit{Vowels}, shows results only on the vowels phonemes. The second column, \textit{Sonorants}, contains the results on the subset which includes vowels, glides, liquids, and nasals phonemes. The last column, shows results on all the phonemes. Note that the results in column \textit{All} for \algoname~and \hubert~are the same results as in Table \ref{tab:results_model1}.


% The last subset, which was used for the results in the previous section, shows results on all the phonemes.
% % and denoted as \textit{All}. 

\algoname~received the best recall and F1 scores, while Kane \emph{et al.} \cite{kane2013improved} received the best precision scores.
% Additionally, better than all the other models, including  \hubert.
Kane \emph{et al.}'s low recall suggests that the high precision is due to miss detection bias. In addition, Praat baseline outperformed Kane \emph{et al.} \cite{kane2013improved} on the \textit{Vowels} and \textit{Sonorants} subsets. Still, Praat baseline's precision score dramatically decreased when evaluated on all phonemes. That demonstrates this model's confusion between voiceless and creaky frames.


\subsubsection{Testing on unseen data}
Finally, we tested our models on the \textit{Prenuclear} and \textit{ALLSSTAR} datasets, which differ from the \textit{Nuclear} dataset we trained on. Both the \textit{Nuclear} and the \textit{Prenuclear} datasets have the same lexical content. However, the \textit{Prenuclear} and \textit{ALLSSTAR} datasets have a different set of speakers and phonetic realizations. Furthermore, the \textit{ALLSSTAR} dataset also has a different lexical content. 

Results are shown in Table \ref{tab:unseen}. It can be seen that in terms of F1 score, \hubert~outperformed the other methods across all datasets. However, Kane \emph{et al.}'s precision is the highest precision on the \textit{Vowels} and \textit{Sonorants}, which is consistent with the results reported in Table \ref{tab:compare_nuc}. Additionally, compared to Table \ref{tab:compare_nuc}, Praat baseline algorithm recall and F1 scores drop.
It is evident that \hubert~ achieved higher F1 and recall scores than \algoname~, still the results of \algoname~are relatively higher than the other methods we compared to. Nevertheless, we note that \hubert~was pre-trained on 960 hours, which is much more data than the 24 minutes of the \textit{Nuclear} dataset we trained \algoname~on. Furthermore, \hubert~has 95M parameters, compared to \algoname~which has less than 5M parameters. Therefore, we believe that training on more data, will improve the results of \algoname.
% Therefore, we believe that \algoname~is still comparable to \hubert~and training on more data, will most likely improve the results of \algoname on unseen data.



==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/intro_nouse.tex <==

\section{Introduction}

Creaky Voice, also known as Vocal fry, is a type of phonation employed across a wide variety of languages with different linguistic and extralinguistic functions. A typical creaky voice has a low rate of vocal fold vibration (pitch), irregular pitch, and constricted glottis, characterized by a small peak glottal opening, long closed phase, and low glottal airflow \cite{keating2015acoustic}. Keating \emph{et al.} \cite{keating2015acoustic} outline several kinds of creaky voice, each of which manifests a slightly different set of acoustic properties. 

% Its role
Cross-linguistically, creaky phonation plays many phonological roles \cite{davidson2021versatility}. It can serve as an utterance-final marker, signal phonemic contrasts with other voice qualities, or be an additional acoustic cue to enhance different contrasts, such as tone (as in Mandarin or Cantonese) \cite{yu2010laryngealization, kuang2017creaky}. It is used as a variant of glottal stop in many languages. Creaky phonation also plays a role in social interaction: it can indicate the end of a conversational turn (Finnish) \cite{ogden2001turn}, indicate an irritation (Vietnamese) \cite{mixdorff2003quantitative}, and be a marker to establish identities \cite{davidson2021versatility}. 

Creaky voice challenges automatic speech processing algorithms due to its irregular periodicity. As a result, algorithms for pitch tracking, spectral analysis, speaker verification, and automatic speech recognition might fail to operate in their full capacity \cite{cullen2013creaky, keshet2018automatic}. This is also a challenge in automatic processing of corpus phonetic and phonological analyses \cite{goldrick2016automatic, chodroff2017structure, chodroff2018corpus}. We believe the community will benefit from an open-source tool for automatic creak detection.

%We follow the footsteps of previous work, which provided automatic tools for phonological analysis as well as corpus phonetic,we release an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians. 

%Previous solutions to such problems were solved by automatic systems for phonological analysis as well as corpus phonetic. Following these recent work and aimed at advancing these fronts, we release/provide an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians.

There have been several studies on algorithms for the detection of creaky voice. Early methods to detect creaky voice were based on ad-hoc signal processing techniques. Vishnubhotla and Espy-Wilson \cite{vishnubhotla2006automatic} proposed a set of rules on the AMDF measure of periodicity. Ishi \emph{et al.} \cite{ishi2007method} suggested to represent the speech by a pulse-synchronized analysis and then use a comparison of intra-frame periodicity and inter-pulse similarity. 

Kane, Drugman, Gobl \emph{et al.} \cite{cullen2013creaky, drugman2012resonator, scherer2013investigating, kane2013improved, drugman2014data} proposed several algorithms which are all based on specially designed acoustic features from the excitation and residual of the linear prediction filtering analysis of the speech and other acoustic features. This line of work used decision trees, fuzzy-input fuzzy-output support vector machine (F$^2$SVM) algorithm, and shallow artificial neural networks for the task. 
Recent work has proposed more advanced learning algorithms, but have been designed for a unique and small data set. Tavi {et al.} \cite{tavi2019recognition} suggested an exploratory creak recognizer based on a convolutional neural network (CNN), which is generated specifically for emergency calls. Villegas \emph{el al.} \cite{villegas2019prediction} used recurrent neural networks to detect creaky of single words in Burmese. 
% \todo{why we didn't compare to other baselines? we should mention here? or in the baselines section?}\\



In contrast to previous work, we propose a deep learning model to detect creaky voice directly from an unprocessed speech signal. % changed fluent to standard connected
The model is built from an encoder and a multi-headed classifier trained together. The encoder is a CNN that takes the raw waveform and learns a representation of the signal. The classifier is a fully-connected network that gets as input the representation and outputs a detection score for creaky voice along with two additional auxiliary tasks: voicing and pitch. These additional predictions steer the overall network toward a better solution in detecting creaky voice \cite{shrem2019dr}.

We use two types of encoders. The first encoder is a specially designed encoder with a large time-span processing window proposed in \cite{segal2021pitch}. It has a larger receptive field than the standard receptive field used in speech processing, and is able to ``see'' several pitch periods, even for very low pitch values. Therefore, we believe that this encoder can contribute to the task of creaky voice detection. This is particularly useful compared to methods that operate on a processed windowed signal (such as MFCC, STFT, and others) and might lose pitch information crucial for identifying creak. 

% which operate with a processed windowed signal (such as MFCC, STFT and others), that might lose pitch information which is crucial for identifying creak. 

The second encoder is based on a state-of-the-art self-supervised representation of the speech called HuBERT \cite{hsu2021hubert} that yields state-of-the-art results for downstream tasks, such as automatic speech recognition \cite{baevski2020wav2vec, hsu2021hubert2}. The latter encoder was pre-trained on 960 hours of read speech. The same multi-headed classifier was used in both models.
 
%is based anon the concept of multi-task learning (MTL). MTL optimizes multiple tasks simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.
% In MTL, multiple related tasks are being optimized simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.

%Additionally, it was previously shown that MTL reduces overfitting while improving generalization all-together. Due to the success of MTL in various fields such as object-detection \cite{ren2015faster, misra2016cross}, natural language processing \cite{collobert2008unified}, speech processing {shrem2019dr}, we perform MTL by encorportaing two additional tasks to the main task of creak detection. \todo{the following is already explained in models-sec3}The first task, identifies if a a given frame is voiced or unvoiced (we label a frame as unvoiced if the phoneme in it is fricatives or consonants). The second task, detects if there was pitch in the frame. We also preform ablation experiments and show that each task helps the final task to improve.

%Our second method is based on the same encoder as the first model, but it is refined using Barlow Twin embedding \cite{zbontar2021barlow}. This method is aimed at maximizing the auto-correlation between the embedding of two augmented variations of a given input. Since it does not require labels, it is a self-supervised learning (SSL) model. Here we exploit this method and use it in the supervised fashion as a method to generate a more refined representation of the signal. 


%The third model is based on the HuBERT model \cite{hsu2021hubert}. This model is a self-supervised representation of the speech. It is a large CNN model trained with a masked prediction task similar to BERT to distinguish subsequent from random future samples \cite{devlin2019bert}. \todo{EC:I rearranged the preceding sentence -- is it still correct?} The learned SSL representations give state-of-the-art results for downstream tasks with minimal supervised data (e.g., for speech recognition, high performance with 10 minutes of annotated speech and 53K hours of untranscribed speech \cite{baevski2020wav2vec, hsu2021hubert2}).\todo{I'm not sure I understand what's in the parentheses} Here we adapted the HuBERT embedding by freezing the representation \todo{which representation?} and adding the same classifier that was used in our first method.

% \textbf{WHAT IS VOCAL FRY/CREAK AND WHY DO WE CARE ABOUT IT:} Vocal fry is one of many phonation types; most common phonation type is modal voice;
% Vocal fry has a variety of acoustic/articulatory forms (Keating/Garellek) -- (we're not good at distinguishing them, so uh, we need to mention this, but collapse);
% Used for various linguistic/extralinguistic functions;
% Standardly used in English for marking phrase finality, but increasingly longer stretches of phonation are common in English -- need refs, what has been found on creak in English? Based on our preliminary analysis, it's not clear it's just a female speech thing. We'll now have that data so we can check, but we should look at the lit to find out what has been said.  
% \textbf{PROBLEM INTRODUCTION:} Creaky voice, with its irregular periodicity, is a well-known issue for f0 tracking. For speech scientists, the most common solution to overcoming this issue involves considerable manual intervention.
% While a few proposals have attempted to detect creak automatically, they have had somewhat limited success in practice. (ehh refs?? how good are they? how are we different?)
% \textbf{PROPOSAL/WHAT WE DO:} We present a (series of) novel neural(?) creak detection system(s) and assess their performance on xxx hours of English speech data that have been manually annotated for intervals of modal and creaky voice. 
% \textbf{EVALUATION:} For stretches of individual utterances, we report the F-score which takes into account the match or mismatch between predicted and gold phonation type labels. 
% \textbf{FINDINGS:} The best-performing system achieved an F-score of xxx and an accuracy of xxx. This was xxx (measurement unit) above our rule-based baseline system.

Trained phoneticians annotated two parallel corpora of connected speech each with 32 American English speakers (Datasets 1 and 2) along with a subset of speech from 14 American English speakers in the ALLSSTAR corpus \cite{bradlow2010allsstar}. The models were trained and developed on Dataset 1, and evaluated on Dataset 2 and the ALLSSTAR corpus. 

Results suggest that both models outperform a heuristics-based baseline model and have better F1 and recall values than Kane \emph{et al.} \cite{kane2013improved}. In addition, the model based on the pre-trained HuBERT representation was marginally better than the specially-designed encoder on unseen data. Our code and pre-trained models are publicly available here: \url{https://github.com/bronichern/DeepFry}.

==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/introduction.tex <==

\section{Introduction}\label{sec:intro}

% background to creaky voice;

Vocal fry, also known as Creaky Voice, is a type of phonation employed across a wide variety of languages with different linguistic and extralinguistic functions. A typical creaky voice has a low rate of vocal fold vibration (pitch), irregular pitch, and constricted glottis, characterized by a small peak glottal opening, long closed phase, and low glottal airflow \cite{keating2015acoustic}. Keating \emph{et al.} \cite{keating2015acoustic} outline several kinds of creaky voice, each of which manifests a slightly different set of acoustic properties. 

% Its role
Cross-linguistically, creaky phonation plays many phonological roles \cite{davidson2021versatility}. It can serve as an utterance-final marker, signal phonemic contrasts with other voice qualities, or be an additional acoustic cue to enhance different contrasts, such as tone (as in Mandarin or Cantonese) \cite{yu2010laryngealization, kuang2017creaky}. It is used as a variant of glottal stop in many languages. Creaky phonation also plays a role in social interaction: it can indicate the end of a conversational turn (Finnish) \cite{ogden2001turn}, indicate an irritation (Vietnamese) \cite{mixdorff2003quantitative}, and be a marker to establish identities \cite{davidson2021versatility}. 

%Historically, creaky voice was associated with upper-class male speakers of Received Pronunciation of British English \cite{dallaston2020quantitative}. Currently, it is increasingly prevalent in English speech, particularly in American English and among young females and celebrities, commonly referred to as a ``language fad,'' or ``vocal pandemic.''\footnote{An article by Marissa Fessenden, ``'Vocal Fry' Creeping Into U.S. Speech'' published on December 9, 2011 at ScienceNOW became one of the most popular articles ever published on the site.}\todo{but debatable whether it is restricted to female/celebrity speech; also common across all speakers, regardless of gender -- but maybe limited to Gen Z/younger millenials}
%\todo{Yossi: Right. Maybe just rewrite this paragraph altogether}

% The problem
Creaky voice challenges automatic speech processing algorithms due to its irregular periodicity. As a result, algorithms for pitch tracking, spectral analysis, speaker verification, and automatic speech recognition might fail to operate in their full capacity \cite{cullen2013creaky, keshet2018automatic}. This is also a challenge in automatic processing of corpus phonetic and phonological analyses \cite{goldrick2016automatic, chodroff2017structure, chodroff2018corpus, hall2019phonological}. We believe the community will benefit from an open-source tool for automatic creak detection.

%We follow the footsteps of previous work, which provided automatic tools for phonological analysis as well as corpus phonetic,we release an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians. 

%Previous solutions to such problems were solved by automatic systems for phonological analysis as well as corpus phonetic. Following these recent work and aimed at advancing these fronts, we release/provide an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians.


There have been several studies on algorithms for the detection of creaky voice. Early methods to detect creaky voice were based on ad-hoc signal processing techniques. Vishnubhotla and Espy-Wilson \cite{vishnubhotla2006automatic} proposed a set of rules on the AMDF measure of periodicity. Ishi \emph{et al.} \cite{ishi2007method} suggested to represent the speech by a pulse-synchronized analysis and then use a comparison of intra-frame periodicity and inter-pulse similarity. 

Kane, Drugman, Gobl \emph{et al.} \cite{cullen2013creaky, drugman2012resonator, scherer2013investigating, kane2013improved, drugman2014data} proposed several algorithms which are all based on specially designed acoustic features from the excitation and residual of the linear prediction filtering analysis of the speech and other acoustic features. This line of work used decision trees, fuzzy-input fuzzy-output support vector machine (F$^2$SVM) algorithm, and shallow artificial neural networks for the task. 
Recent work has proposed more advanced learning algorithms, but have been designed for a unique and small data set. Tavi {et al.} \cite{tavi2019recognition} suggested an exploratory creak recognizer based on a convolutional neural network (CNN), which is generated specifically for emergency calls. Villegas \emph{el al.} \cite{villegas2019prediction} used recurrent neural networks to detect creaky of single words in Burmese.

In contrast to previous work, we propose a deep learning model to detect creaky voice directly from an unprocessed speech signal. % changed fluent to standard connected
The model is built from an encoder and a multi-headed classifier trained together. The encoder is a CNN that takes the raw waveform and learns a representation of the signal. The classifier is a fully-connected network that gets as input the representation and outputs a detection score for creaky voice along with two additional auxiliary tasks: voicing and pitch. These additional predictions steer the overall network toward a better solution in detecting creaky voice \cite{shrem2019dr}.

We use two types of encoders. The first encoder is a specially designed encoder with a large time-span processing window proposed in \cite{segal2021pitch}. It has a larger receptive field than the standard receptive field used in speech processing, and is able to ``see'' several pitch periods, even for very low pitch values. Therefore, we believe that this encoder can contribute to the task of creaky voice detection. This is particularly useful compared to methods that operate on a processed windowed signal (such as MFCC, STFT, and others) and might lose pitch information crucial for identifying creak. 
% which operate with a processed windowed signal (such as MFCC, STFT and others), that might lose pitch information which is crucial for identifying creak. 

The second encoder is based on a state-of-the-art self-supervised representation of the speech called HuBERT \cite{hsu2021hubert} that yields state-of-the-art results for downstream tasks, such as automatic speech recognition \cite{baevski2020wav2vec, hsu2021hubert2}. The latter encoder was pre-trained on 960 hours of read speech. The same multi-headed classifier was used in both models.
 
%is based anon the concept of multi-task learning (MTL). MTL optimizes multiple tasks simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.
% In MTL, multiple related tasks are being optimized simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.

%Additionally, it was previously shown that MTL reduces overfitting while improving generalization all-together. Due to the success of MTL in various fields such as object-detection \cite{ren2015faster, misra2016cross}, natural language processing \cite{collobert2008unified}, speech processing {shrem2019dr}, we perform MTL by encorportaing two additional tasks to the main task of creak detection. \todo{the following is already explained in models-sec3}The first task, identifies if a a given frame is voiced or unvoiced (we label a frame as unvoiced if the phoneme in it is fricatives or consonants). The second task, detects if there was pitch in the frame. We also preform ablation experiments and show that each task helps the final task to improve.

%Our second method is based on the same encoder as the first model, but it is refined using Barlow Twin embedding \cite{zbontar2021barlow}. This method is aimed at maximizing the auto-correlation between the embedding of two augmented variations of a given input. Since it does not require labels, it is a self-supervised learning (SSL) model. Here we exploit this method and use it in the supervised fashion as a method to generate a more refined representation of the signal. 


%The third model is based on the HuBERT model \cite{hsu2021hubert}. This model is a self-supervised representation of the speech. It is a large CNN model trained with a masked prediction task similar to BERT to distinguish subsequent from random future samples \cite{devlin2019bert}. \todo{EC:I rearranged the preceding sentence -- is it still correct?} The learned SSL representations give state-of-the-art results for downstream tasks with minimal supervised data (e.g., for speech recognition, high performance with 10 minutes of annotated speech and 53K hours of untranscribed speech \cite{baevski2020wav2vec, hsu2021hubert2}).\todo{I'm not sure I understand what's in the parentheses} Here we adapted the HuBERT embedding by freezing the representation \todo{which representation?} and adding the same classifier that was used in our first method.

% \textbf{WHAT IS VOCAL FRY/CREAK AND WHY DO WE CARE ABOUT IT:} Vocal fry is one of many phonation types; most common phonation type is modal voice;
% Vocal fry has a variety of acoustic/articulatory forms (Keating/Garellek) -- (we're not good at distinguishing them, so uh, we need to mention this, but collapse);
% Used for various linguistic/extralinguistic functions;
% Standardly used in English for marking phrase finality, but increasingly longer stretches of phonation are common in English -- need refs, what has been found on creak in English? Based on our preliminary analysis, it's not clear it's just a female speech thing. We'll now have that data so we can check, but we should look at the lit to find out what has been said.  
% \textbf{PROBLEM INTRODUCTION:} Creaky voice, with its irregular periodicity, is a well-known issue for f0 tracking. For speech scientists, the most common solution to overcoming this issue involves considerable manual intervention.
% While a few proposals have attempted to detect creak automatically, they have had somewhat limited success in practice. (ehh refs?? how good are they? how are we different?)
% \textbf{PROPOSAL/WHAT WE DO:} We present a (series of) novel neural(?) creak detection system(s) and assess their performance on xxx hours of English speech data that have been manually annotated for intervals of modal and creaky voice. 
% \textbf{EVALUATION:} For stretches of individual utterances, we report the F-score which takes into account the match or mismatch between predicted and gold phonation type labels. 
% \textbf{FINDINGS:} The best-performing system achieved an F-score of xxx and an accuracy of xxx. This was xxx (measurement unit) above our rule-based baseline system.

Trained phoneticians annotated two parallel corpora of connected speech each with 32 American English speakers (Datasets 1 and 2) along with a subset of speech from 14 American English speakers in the ALLSSTAR corpus \cite{bradlow2010allsstar}. The models were trained and developed on Dataset 1, and evaluated on Dataset 2 and the ALLSSTAR corpus. 

Results suggest that both models outperform a heuristics-based baseline model and have better F1 and recall values than Kane \emph{et al.} \cite{kane2013improved}. In addition, the model based on the pre-trained HuBERT representation was marginally better than the specially-designed encoder on unseen data. Our code and pre-trained models are publicly available here: {\footnotesize \url{https://github.com/bronichern/DeepFry}}.

==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/models.tex <==
%\section{Models description}\label{sec:models}
\section{Method}
\label{sec:models}

The input to all models is the raw waveform. Formally, we denote a speech waveform of $T$ samples by $\bar{x}=(x_1,\ldots,x_T)$, where $x_t\in\X$ for $t\in[1, T]$ and $\X\subseteq\reals$. Our setting is designed to allow different input duration hence $T$ is not fixed.  
%The waveform is represented in the models as a sequence of $K$ overlapping frames, where each frame span $m$ samples, with an overlap of $n$ samples. We denote each frame by $\x_k\in\X$, where $\X\subseteq\reals^m$. Denote the sequence of frames by $\sx  = (\x_1,\ldots,\x_K)$. 
We assume that there is a sequence of $K$ multi-labels, $\sy = (y_1,\ldots,y_K)$, where each multi-label $y_k$ is from the set $\Y = \{\text{(creaky, not-creaky), (voiced,unvoiced), (pitch,no-pitch)}\}$. %$\sy_{k}^i\in \Y^i$, such that 
% $\sy_{ik}\in \Y^{(1,3)}=\{\text{creaky, not-creaky}\}$ is the label of the $k$-th frame.

Our models are composed of two neural networks. The \emph{encoder} $g: \X\to \Z^K$ is a function from the domain of $\X$ to the embedding space $\Z \subseteq \reals^N$. Specifically, the encoder generates a sequence of representational vectors $\sz  = (z_1,\ldots,z_K)$, where $z_k \in \Z$, for all $1 \leq k \leq K$, such that $z_k\in\Z$ is the acoustic embedding of the $k$-th frame. The embeddings are then processed by a classifier that outputs a sequence of $K$ predictions. The \emph{classifier} is a function $f: \Z^K\to \Y^K$ from the domain of features vectors to the domain of target objects. 
% \todo{update with center \& size} 
Figure~\ref{fig:architecture} depicts an encoder and the multi-headed classifier. The encoder $g$ is a fully convolutional neural network and is based on the framework proposed in \cite{segal2021pitch} for pitch estimation. This encoder gets as input a variable duration signal and outputs a sequence of embedding vectors every 5 msec (due to hardware limitations, the number of embedding vectors was restricted to less than 100 per input). It has a larger receptive field than the standard receptive field used in speech processing, and therefore can handle several pitch periods. We denoted this encoder-classifier combination as \algoname. 
% We believe that it can contribute to the task of creaky voice detection, especially compared to methods which operate with a processed windowed signal (such as MFCC, STFT and others), which might lose pitch information which is crucial for identifying creak. 

% We believe that this encoder can contribute to the task of creaky voice detection, since it works on the raw waveform and has a larger receptive field than the standard receptive field used in speech processing. This is particularly useful compared to methods which operate with a processed windowed signal (such as MFCC, STFT and others), that might lose pitch information which is crucial for identifying creak. 

In our work we also use another encoder which is based on the HuBERT model \cite{hsu2021hubert}. This model learns a representation of the speech in a self-supervised manner. It is a large CNN model trained to distinguish a series of subsequent samples from random future samples when some representations are masked, similar to the BERT model \cite{devlin2019bert}. The rationale behind this concept is that subsequent samples are more likely to belong to the same phonetic class than random future samples. Here we used the HuBERT model that was pre-trained on 960 hours of read speech (LibriSpeech). The model operates on a 20 ms frame-rate window.  We denoted this encoder-classifier combination as \hubert. 

Our classifier is based on the concept of multi-task learning (MTL). MTL optimizes multiple tasks simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.  Specifically our classifier $f$ is aimed at detecting creaky voice (binary),  voice/unvoiced (binary) and pitch (binary). The voiced/unvoiced was annotated by expert phoneticians, and the pitch was extracted using \cite{boersma1993accurate}.

%\todo{THIS SHOULD BE IN DATASET:}We also relabel the creaky labels during training, such that if a segment is unvoiced, the label is set to not-creak. \\
% Binary classification of whether the pitch is 0 or not
% If the pitch is 0, below 200, above 200.
% will be one of tohse

\begin{figure}[h]
 \centering
% \includegraphics[width=1.1\linewidth, height=0.4\textwidth]{layers2.pdf}
\includegraphics[width=\linewidth]{layers2.1.pdf}
 \vspace{-0.7cm}
 \caption{Model architecture. The encoder has 5 CNN layers, and the classifier has 2 fully-connected layers with 3 classification heads: creaky, voiced, pitch.}
 \label{fig:architecture}
\end{figure}

% We now turn to describe each model in detail.
% \subsection{Model 1: Base \todo{name it diff.}}

% \subsection{Model 2: Barlow-Twins with fine-tuning}
% The second model attempts to improve the learned representation, by using a Self-Supervised Learning (SSL) method. First, operating on 5 ms frame-rate window, we train a Barlow-Twins framework \cite{zbontar2021barlow}, using the encoder mentioned above, without a projection layer. Also, instead of performing transformations on a single input, we present two instances of creak, or two non-creak instances, where the instances are from different speakers. We trained the model using the optimization of \cite{zbontar2021barlow} but with a learning rate of 0.002. After convergence, we use the weights of the model to initialize and train Model 1.

% \subsection{Model 2 - Hubert with fine-tuning}
% \todo{SSL models \& success will be written in the intro, don't think it's relevant here}
% SSL has shown great success in capturing signal properties, therefore we use a pre-trained Hubert \cite{hsu2021hubert} which is SSL state-of-art system as the encoder of our system and freeze its weights. 
% The model operates on a 20 ms frame-rate window. \todo{FILLOUT TRAINING}
% % We used the HuBERT pri-traind Base model published by fairseq to extract the HuBERT feature.
% Using the classifier mentioned above with input size of 768,  \\\\


% The third model also utilizes SSL and uses a pre-trained Hubert \cite{hsu2021hubert} as the encoder. To do so, we keep the weights fixed and only train the classifier. The model operates on a 20 ms frame-rate window. Additionally, we change the first layer of the classifier to receive an input size of 768 instead of 512 in the original classifier. The model was trained for six epochs, with an Adam optimizer, a learning rate of 0.001, and a batch size of 16.




==> DeepFry_ Identifying Creaky Voice From Raw Speech Signal/problem_settings.tex <==
% !TEX root =  main.tex

\section{Method}
\label{sec:models}

The input to all models is the raw waveform. Formally, we denote a speech waveform of $T$ samples by $\bar{x}=(x_1,\ldots,x_T)$, where $x_t\in\X$ for $t\in[1, T]$ and $\X\subseteq\reals$. Our setting is designed to allow different input duration hence $T$ is not fixed.  
%The waveform is represented in the models as a sequence of $K$ overlapping frames, where each frame span $m$ samples, with an overlap of $n$ samples. We denote each frame by $\x_k\in\X$, where $\X\subseteq\reals^m$. Denote the sequence of frames by $\sx  = (\x_1,\ldots,\x_K)$. 
We assume that there is a sequence of $K$ multi-labels, $\sy = (y_1,\ldots,y_K)$, where each multi-label $y_k$ is from the set $\Y = \{\text{(creaky, not-creaky), (voiced,unvoiced), (pitch,no-pitch)}\}$. %$\sy_{k}^i\in \Y^i$, such that 
% $\sy_{ik}\in \Y^{(1,3)}=\{\text{creaky, not-creaky}\}$ is the label of the $k$-th frame.

Our models are composed of two neural networks. The \emph{encoder} $g: \X\to \Z^K$ is a function from the domain of $\X$ to the embedding space $\Z \subseteq \reals^N$. Specifically, the encoder generates a sequence of representational vectors $\sz  = (z_1,\ldots,z_K)$, where $z_k \in \Z$, for all $1 \leq k \leq K$, such that $z_k\in\Z$ is the acoustic embedding of the $k$-th frame. The embeddings are then processed by a classifier that outputs a sequence of $K$ predictions. The \emph{classifier} is a function $f: \Z^K\to \Y^K$ from the domain of features vectors to the domain of target objects. 


% The functions $g$ and $f$ are implemented using deep learning functions by two models. The first model is depicted in the top panel of Figure~\ref{fig:architectures}. In this model, a convolutional neural network (CNN) is used as a features extraction function, $g$. It has five 1D convolutional layers with batch normalization, a leaky-ReLU activation function, and dropout between each layer. The features extractor output is then forwarded to the classifier $f$, composed of a two-layer bi-directional long short-term memory (LSTM) and two fully-connected (FC) layers. This model will be denoted as \emph{\lstm}. 

% The second model is depicted in the bottom panel of Figure~\ref{fig:architectures}. In recent work, it has been suggested that CNN architectures are an effective replacement of recurrent models \cite{collobert2016wav2letter}, and we exploit this idea in our models. In our second model, a CNN architecture is used for the feature extraction function $g$ and the classifier function $f$. It has ten 1D convolutional layers with batch normalization, a leaky-ReLU activation function, and dropout between each layer. The output of the CNN is forwarded to two FC layers. This model will be denoted as \emph{\cnn}.

% The parameters of both models are trained to minimize the cross-entropy loss function. For both models, a \emph{post-processing procedure} is used to convert the frame-based to segment-based predictions. First, we group together frames with the same object type.



% \section{Problem Setting}
% %DESCRPTION OF METHOD....
% To identify creak, we operate on the raw wave sampled at 16 kHz.
% Formally, denote a speech utterance of $T$ samples by $\sx  = (x_1,\ldots,x_T)$, where $x_t\in\X$ for all $1 \leq t \leq T$ and $\X \subset \reals $. We represent the output as a sequence of $m$ \todo{this varies between models} milliseconds frames, $\sy = (y_1,\ldots,y_K)$ for  $1 \leq k \leq K$,  where each frame $y_k\in \Y=\{\text{creaky, not-creaky}\}$ . Note that the signal duration $T$ and the number of output frames $k$ can vary from one signal to another, and thus these quantities are not fixed. 

% \todo{very similar to the ddk paper- should we change it?}
% Our models are composed of two neural networks. The \emph{encoder} $g: \X\to \Z^K$ is a function from the domain of $\X$ to the embedding space $\Z \subseteq \reals^N$. Specifically, the encoder generates a sequence of representational vectors $\sz  = (z_1,\ldots,z_K)$, where $z_k \in \Z$, for all $1 \leq k \leq K$, such that $z_k\in\Z$ is the acoustic representation of the $k$-th frame.
% The feature vector sequence is then processed by a classifier that outputs a sequence of $K$ predictions. The \emph{classifier} $f: \Z^K\to \Y^K$ from the domain of features vectors to the domain of target objects.
% \todo {adjust the commented sections per final depicted model}



==> LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> bibtoadd.tex <==


@article{ishi2007method,
  title={A method for automatic detection of vocal fry},
  author={Ishi, Carlos Toshinori and Sakakibara, Ken-Ichi and Ishiguro, Hiroshi and Hagita, Norihiro},
  journal={IEEE transactions on audio, speech, and language processing},
  volume={16},
  number={1},
  pages={47--56},
  year={2007},
  publisher={IEEE}
}

@article{kane2013improved,
  title={Improved automatic detection of creak},
  author={Kane, John and Drugman, Thomas and Gobl, Christer},
  journal={Computer Speech \& Language},
  volume={27},
  number={4},
  pages={1028--1047},
  year={2013},
  publisher={Elsevier}
}

%%%%checking code
@inproceedings{white2021optimizing,
  title={Optimizing an automatic creaky voice detection method for Australian English-speaking females},
  author={White, Hannah and Penney, Joshua and Gibson, Andy and Szakay, Anita and Cox, Felicity},
  booktitle={INTERSPEECH (22nd: 2021)},
  pages={1384--1388},
  year={2021},
  organization={International Speech Communication Association (ISCA)}
}

@article{devaraj2021modelling,
  title={Modelling of Amplitude Modulated Vocal Fry Glottal Area Waveforms Using an Analysis-by-Synthesis Approach},
  author={Devaraj, Vinod and Aichinger, Philipp},
  journal={Applied Sciences},
  volume={11},
  number={5},
  pages={1990},
  year={2021},
  publisher={Multidisciplinary Digital Publishing Institute}
}

==> intro_nouse.tex <==

\section{Introduction}

Creaky Voice, also known as Vocal fry, is a type of phonation employed across a wide variety of languages with different linguistic and extralinguistic functions. A typical creaky voice has a low rate of vocal fold vibration (pitch), irregular pitch, and constricted glottis, characterized by a small peak glottal opening, long closed phase, and low glottal airflow \cite{keating2015acoustic}. Keating \emph{et al.} \cite{keating2015acoustic} outline several kinds of creaky voice, each of which manifests a slightly different set of acoustic properties. 

% Its role
Cross-linguistically, creaky phonation plays many phonological roles \cite{davidson2021versatility}. It can serve as an utterance-final marker, signal phonemic contrasts with other voice qualities, or be an additional acoustic cue to enhance different contrasts, such as tone (as in Mandarin or Cantonese) \cite{yu2010laryngealization, kuang2017creaky}. It is used as a variant of glottal stop in many languages. Creaky phonation also plays a role in social interaction: it can indicate the end of a conversational turn (Finnish) \cite{ogden2001turn}, indicate an irritation (Vietnamese) \cite{mixdorff2003quantitative}, and be a marker to establish identities \cite{davidson2021versatility}. 

Creaky voice challenges automatic speech processing algorithms due to its irregular periodicity. As a result, algorithms for pitch tracking, spectral analysis, speaker verification, and automatic speech recognition might fail to operate in their full capacity \cite{cullen2013creaky, keshet2018automatic}. This is also a challenge in automatic processing of corpus phonetic and phonological analyses \cite{goldrick2016automatic, chodroff2017structure, chodroff2018corpus}. We believe the community will benefit from an open-source tool for automatic creak detection.

%We follow the footsteps of previous work, which provided automatic tools for phonological analysis as well as corpus phonetic,we release an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians. 

%Previous solutions to such problems were solved by automatic systems for phonological analysis as well as corpus phonetic. Following these recent work and aimed at advancing these fronts, we release/provide an open-source tool for automatic creak detection that will particularly benefit the community of phoneticians.

There have been several studies on algorithms for the detection of creaky voice. Early methods to detect creaky voice were based on ad-hoc signal processing techniques. Vishnubhotla and Espy-Wilson \cite{vishnubhotla2006automatic} proposed a set of rules on the AMDF measure of periodicity. Ishi \emph{et al.} \cite{ishi2007method} suggested to represent the speech by a pulse-synchronized analysis and then use a comparison of intra-frame periodicity and inter-pulse similarity. 

Kane, Drugman, Gobl \emph{et al.} \cite{cullen2013creaky, drugman2012resonator, scherer2013investigating, kane2013improved, drugman2014data} proposed several algorithms which are all based on specially designed acoustic features from the excitation and residual of the linear prediction filtering analysis of the speech and other acoustic features. This line of work used decision trees, fuzzy-input fuzzy-output support vector machine (F$^2$SVM) algorithm, and shallow artificial neural networks for the task. 
Recent work has proposed more advanced learning algorithms, but have been designed for a unique and small data set. Tavi {et al.} \cite{tavi2019recognition} suggested an exploratory creak recognizer based on a convolutional neural network (CNN), which is generated specifically for emergency calls. Villegas \emph{el al.} \cite{villegas2019prediction} used recurrent neural networks to detect creaky of single words in Burmese. 
% \todo{why we didn't compare to other baselines? we should mention here? or in the baselines section?}\\



In contrast to previous work, we propose a deep learning model to detect creaky voice directly from an unprocessed speech signal. % changed fluent to standard connected
The model is built from an encoder and a multi-headed classifier trained together. The encoder is a CNN that takes the raw waveform and learns a representation of the signal. The classifier is a fully-connected network that gets as input the representation and outputs a detection score for creaky voice along with two additional auxiliary tasks: voicing and pitch. These additional predictions steer the overall network toward a better solution in detecting creaky voice \cite{shrem2019dr}.

We use two types of encoders. The first encoder is a specially designed encoder with a large time-span processing window proposed in \cite{segal2021pitch}. It has a larger receptive field than the standard receptive field used in speech processing, and is able to ``see'' several pitch periods, even for very low pitch values. Therefore, we believe that this encoder can contribute to the task of creaky voice detection. This is particularly useful compared to methods that operate on a processed windowed signal (such as MFCC, STFT, and others) and might lose pitch information crucial for identifying creak. 

% which operate with a processed windowed signal (such as MFCC, STFT and others), that might lose pitch information which is crucial for identifying creak. 

The second encoder is based on a state-of-the-art self-supervised representation of the speech called HuBERT \cite{hsu2021hubert} that yields state-of-the-art results for downstream tasks, such as automatic speech recognition \cite{baevski2020wav2vec, hsu2021hubert2}. The latter encoder was pre-trained on 960 hours of read speech. The same multi-headed classifier was used in both models.
 
%is based anon the concept of multi-task learning (MTL). MTL optimizes multiple tasks simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.
% In MTL, multiple related tasks are being optimized simultaneously, under the assumption that the information shared by they task will help boost the performance of the model on the task of interest.

%Additionally, it was previously shown that MTL reduces overfitting while improving generalization all-together. Due to the success of MTL in various fields such as object-detection \cite{ren2015faster, misra2016cross}, natural language processing \cite{collobert2008unified}, speech processing {shrem2019dr}, we perform MTL by encorportaing two additional tasks to the main task of creak detection. \todo{the following is already explained in models-sec3}The first task, identifies if a a given frame is voiced or unvoiced (we label a frame as unvoiced if the phoneme in it is fricatives or consonants). The second task, detects if there was pitch in the frame. We also preform ablation experiments and show that each task helps the final task to improve.

%Our second method is based on the same encoder as the first model, but it is refined using Barlow Twin embedding \cite{zbontar2021barlow}. This method is aimed at maximizing the auto-correlation between the embedding of two augmented variations of a given input. Since it does not require labels, it is a self-supervised learning (SSL) model. Here we exploit this method and use it in the supervised fashion as a method to generate a more refined representation of the signal. 


%The third model is based on the HuBERT model \cite{hsu2021hubert}. This model is a self-supervised representation of the speech. It is a large CNN model trained with a masked prediction task similar to BERT to distinguish subsequent from random future samples \cite{devlin2019bert}. \todo{EC:I rearranged the preceding sentence -- is it still correct?} The learned SSL representations give state-of-the-art results for downstream tasks with minimal supervised data (e.g., for speech recognition, high performance with 10 minutes of annotated speech and 53K hours of untranscribed speech \cite{baevski2020wav2vec, hsu2021hubert2}).\todo{I'm not sure I understand what's in the parentheses} Here we adapted the HuBERT embedding by freezing the representation \todo{which representation?} and adding the same classifier that was used in our first method.

% \textbf{WHAT IS VOCAL FRY/CREAK AND WHY DO WE CARE ABOUT IT:} Vocal fry is one of many phonation types; most common phonation type is modal voice;
% Vocal fry has a variety of acoustic/articulatory forms (Keating/Garellek) -- (we're not good at distinguishing them, so uh, we need to mention this, but collapse);
% Used for various linguistic/extralinguistic functions;
% Standardly used in English for marking phrase finality, but increasingly longer stretches of phonation are common in English -- need refs, what has been found on creak in English? Based on our preliminary analysis, it's not clear it's just a female speech thing. We'll now have that data so we can check, but we should look at the lit to find out what has been said.  
% \textbf{PROBLEM INTRODUCTION:} Creaky voice, with its irregular periodicity, is a well-known issue for f0 tracking. For speech scientists, the most common solution to overcoming this issue involves considerable manual intervention.
% While a few proposals have attempted to detect creak automatically, they have had somewhat limited success in practice. (ehh refs?? how good are they? how are we different?)
% \textbf{PROPOSAL/WHAT WE DO:} We present a (series of) novel neural(?) creak detection system(s) and assess their performance on xxx hours of English speech data that have been manually annotated for intervals of modal and creaky voice. 
% \textbf{EVALUATION:} For stretches of individual utterances, we report the F-score which takes into account the match or mismatch between predicted and gold phonation type labels. 
% \textbf{FINDINGS:} The best-performing system achieved an F-score of xxx and an accuracy of xxx. This was xxx (measurement unit) above our rule-based baseline system.

Trained phoneticians annotated two parallel corpora of connected speech each with 32 American English speakers (Datasets 1 and 2) along with a subset of speech from 14 American English speakers in the ALLSSTAR corpus \cite{bradlow2010allsstar}. The models were trained and developed on Dataset 1, and evaluated on Dataset 2 and the ALLSSTAR corpus. 

Results suggest that both models outperform a heuristics-based baseline model and have better F1 and recall values than Kane \emph{et al.} \cite{kane2013improved}. In addition, the model based on the pre-trained HuBERT representation was marginally better than the specially-designed encoder on unseen data. Our code and pre-trained models are publicly available here: \url{https://github.com/bronichern/DeepFry}.

==> problem_settings.tex <==
% !TEX root =  main.tex

\section{Method}
\label{sec:models}

The input to all models is the raw waveform. Formally, we denote a speech waveform of $T$ samples by $\bar{x}=(x_1,\ldots,x_T)$, where $x_t\in\X$ for $t\in[1, T]$ and $\X\subseteq\reals$. Our setting is designed to allow different input duration hence $T$ is not fixed.  
%The waveform is represented in the models as a sequence of $K$ overlapping frames, where each frame span $m$ samples, with an overlap of $n$ samples. We denote each frame by $\x_k\in\X$, where $\X\subseteq\reals^m$. Denote the sequence of frames by $\sx  = (\x_1,\ldots,\x_K)$. 
We assume that there is a sequence of $K$ multi-labels, $\sy = (y_1,\ldots,y_K)$, where each multi-label $y_k$ is from the set $\Y = \{\text{(creaky, not-creaky), (voiced,unvoiced), (pitch,no-pitch)}\}$. %$\sy_{k}^i\in \Y^i$, such that 
% $\sy_{ik}\in \Y^{(1,3)}=\{\text{creaky, not-creaky}\}$ is the label of the $k$-th frame.

Our models are composed of two neural networks. The \emph{encoder} $g: \X\to \Z^K$ is a function from the domain of $\X$ to the embedding space $\Z \subseteq \reals^N$. Specifically, the encoder generates a sequence of representational vectors $\sz  = (z_1,\ldots,z_K)$, where $z_k \in \Z$, for all $1 \leq k \leq K$, such that $z_k\in\Z$ is the acoustic embedding of the $k$-th frame. The embeddings are then processed by a classifier that outputs a sequence of $K$ predictions. The \emph{classifier} is a function $f: \Z^K\to \Y^K$ from the domain of features vectors to the domain of target objects. 


% The functions $g$ and $f$ are implemented using deep learning functions by two models. The first model is depicted in the top panel of Figure~\ref{fig:architectures}. In this model, a convolutional neural network (CNN) is used as a features extraction function, $g$. It has five 1D convolutional layers with batch normalization, a leaky-ReLU activation function, and dropout between each layer. The features extractor output is then forwarded to the classifier $f$, composed of a two-layer bi-directional long short-term memory (LSTM) and two fully-connected (FC) layers. This model will be denoted as \emph{\lstm}. 

% The second model is depicted in the bottom panel of Figure~\ref{fig:architectures}. In recent work, it has been suggested that CNN architectures are an effective replacement of recurrent models \cite{collobert2016wav2letter}, and we exploit this idea in our models. In our second model, a CNN architecture is used for the feature extraction function $g$ and the classifier function $f$. It has ten 1D convolutional layers with batch normalization, a leaky-ReLU activation function, and dropout between each layer. The output of the CNN is forwarded to two FC layers. This model will be denoted as \emph{\cnn}.

% The parameters of both models are trained to minimize the cross-entropy loss function. For both models, a \emph{post-processing procedure} is used to convert the frame-based to segment-based predictions. First, we group together frames with the same object type.



% \section{Problem Setting}
% %DESCRPTION OF METHOD....
% To identify creak, we operate on the raw wave sampled at 16 kHz.
% Formally, denote a speech utterance of $T$ samples by $\sx  = (x_1,\ldots,x_T)$, where $x_t\in\X$ for all $1 \leq t \leq T$ and $\X \subset \reals $. We represent the output as a sequence of $m$ \todo{this varies between models} milliseconds frames, $\sy = (y_1,\ldots,y_K)$ for  $1 \leq k \leq K$,  where each frame $y_k\in \Y=\{\text{creaky, not-creaky}\}$ . Note that the signal duration $T$ and the number of output frames $k$ can vary from one signal to another, and thus these quantities are not fixed. 

% \todo{very similar to the ddk paper- should we change it?}
% Our models are composed of two neural networks. The \emph{encoder} $g: \X\to \Z^K$ is a function from the domain of $\X$ to the embedding space $\Z \subseteq \reals^N$. Specifically, the encoder generates a sequence of representational vectors $\sz  = (z_1,\ldots,z_K)$, where $z_k \in \Z$, for all $1 \leq k \leq K$, such that $z_k\in\Z$ is the acoustic representation of the $k$-th frame.
% The feature vector sequence is then processed by a classifier that outputs a sequence of $K$ predictions. The \emph{classifier} $f: \Z^K\to \Y^K$ from the domain of features vectors to the domain of target objects.
% \todo {adjust the commented sections per final depicted model}


